Simultaneous space and phase resolved X-ray polarimetry of the Crab Pulsar and Nebula

The Crab pulsar and its nebula are among the most studied astrophysical systems, and constitute one of the most promising environments where high energy processes and particle acceleration can be investigated. They are the only objects for which previous X-ray polarisation has been reported. We present here the first Imaging X-ray Polarimetry Explorer (IXPE) observation of the Crab pulsar and nebula. The total pulsar pulsed emission in the [2-8] keV energy range is unpolarised. Significant polarisation up to 15% is detected only in the core of the main peak. The nebula has a total space integrated polarised degree of 20% and polarisation angle of 145deg. The polarised maps show a large variation in the local polarisation, and regions with polarised degree up to 45-50%. The polarisation pattern suggests a predominantly toroidal magnetic field.

==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}


